COMBINEX: A Unified Counterfactual Explainer for Graph Neural Networks via Node Feature and Structural Perturbations

Counterfactual explanations have emerged as a powerful tool to unveil the opaque decision-making processes of graph neural networks (GNNs). However, existing techniques primarily focus on edge modifications, often overlooking the crucial role of node feature perturbations in shaping model predictions. To address this limitation, we propose COMBINEX, a novel GNN explainer that generates counterfactual explanations for both node and graph classification tasks. Unlike prior methods, which treat structural and feature-based changes independently, COMBINEX optimally balances modifications to edges and node features by jointly optimizing these perturbations. This unified approach ensures minimal yet effective changes required to flip a model's prediction, resulting in realistic and interpretable counterfactuals. Additionally, COMBINEX seamlessly handles both continuous and discrete node features, enhancing its versatility across diverse datasets and GNN architectures. Extensive experiments on real-world datasets and various GNN architectures demonstrate the effectiveness and robustness of our approach over existing baselines.

==> tables/time_memory/time.tex <==
\begin{table*}
\centering
\begin{tabular}{ccccc}
\hline
 Dataset &  Model & Explainer & Time (s) ($\pm$ std) & Memory (MB) ($\pm$ std) \\
\hline
  citeseer & GCN & CF-GNN & $ 4.708 (\pm 0.259)$ & $ 1423.094 (\pm 109.791)$ \\
  citeseer & GCN & Random F. & $ 1.296 (\pm 0.022)$ & $ 1332.542 (\pm 161.333)$ \\
  citeseer & GCN & Random E. & $ 1.345 (\pm 0.032)$ & $ 1302.075 (\pm 151.000)$ \\
  citeseer & GCN & EGO & $n.a.$ & $n.a.$ \\
  citeseer & GCN & CFF & $n.a.$ & $ 1459.056 (\pm 80.511)$ \\
  citeseer & GCN & Combinex & $ 7.881 (\pm 0.191)$ & $ 1566.162 (\pm 117.538)$ \\
  citeseer & GCN & UNR & $ 0.053 (\pm 0.042)$ & $n.a.$ \\
  protein & GCN & CF-GNN & $n.a.$ & $ 1780.618 (\pm 130.201)$ \\
  protein & GCN & Random F. & $ 1.275 (\pm 0.005)$ & $ 1690.737 (\pm 209.816)$ \\
  protein & GCN & Random E. & $ 1.300 (\pm 0.021)$ & $ 1697.304 (\pm 198.443)$ \\
  protein & GCN & EGO & $n.a.$ & $n.a.$ \\
  protein & GCN & CFF & $ 8.679 (\pm 0.321)$ & $ 1802.785 (\pm 91.550)$ \\
  protein & GCN & Combinex & $ 7.732 (\pm 0.101)$ & $ 1799.258 (\pm 99.061)$ \\
  protein & GCN & UNR & $n.a.$ & $ 1327.325 (\pm 0.000)$ \\
  enzymes & GCN & CF-GNN & $ 4.616 (\pm 0.115)$ & $ 1517.080 (\pm 102.136)$ \\
  enzymes & GCN & Random F. & $ 1.278 (\pm 0.024)$ & $ 1433.129 (\pm 150.961)$ \\
  enzymes & GCN & Random E. & $ 1.331 (\pm 0.009)$ & $ 1459.816 (\pm 138.667)$ \\
  enzymes & GCN & EGO & $ 0.009 (\pm 0.003)$ & $n.a.$ \\
  enzymes & GCN & CFF & $n.a.$ & $ 1536.265 (\pm 65.271)$ \\
  enzymes & GCN & Combinex & $ 7.587 (\pm 0.185)$ & $ 1531.650 (\pm 70.724)$ \\
  enzymes & GCN & UNR & $ 0.102 (\pm 0.173)$ & $ 1221.638 (\pm 0.000)$ \\
  karate & GCN & CF-GNN & $n.a.$ & $ 1077.875 (\pm 0.000)$ \\
  karate & GCN & Random F. & $ 1.230 (\pm 0.010)$ & $n.a.$ \\
  karate & GCN & Random E. & $ 1.485 (\pm 0.212)$ & $n.a.$ \\
  karate & GCN & EGO & $n.a.$ & $n.a.$ \\
  karate & GCN & CFF & $n.a.$ & $ 1209.475 (\pm 132.400)$ \\
  karate & GCN & Combinex & $ 7.923 (\pm 0.234)$ & $ 1209.142 (\pm 130.733)$ \\
  karate & GCN & UNR & $n.a.$ & $n.a.$ \\
  actor & GCN & CF-GNN & $ 4.880 (\pm 0.285)$ & $ 1688.808 (\pm 159.201)$ \\
  actor & GCN & Random F. & $ 1.305 (\pm 0.032)$ & $ 1583.875 (\pm 236.133)$ \\
  actor & GCN & Random E. & $ 1.391 (\pm 0.064)$ & $ 1504.875 (\pm 206.867)$ \\
  actor & GCN & EGO & $ 0.010 (\pm 0.004)$ & $n.a.$ \\
  actor & GCN & CFF & $ 9.062 (\pm 0.237)$ & $ 1690.044 (\pm 118.154)$ \\
  actor & GCN & Combinex & $ 8.066 (\pm 0.357)$ & $ 2275.003 (\pm 259.763)$ \\
  actor & GCN & UNR & $n.a.$ & $ 1204.408 (\pm 0.000)$ \\
  Wiki & GCN & CF-GNN & $ 4.702 (\pm 0.224)$ & $ 1613.808 (\pm 163.273)$ \\
  Wiki & GCN & Random F. & $ 1.255 (\pm 0.006)$ & $ 1978.631 (\pm 511.389)$ \\
  Wiki & GCN & Random E. & $ 1.384 (\pm 0.016)$ & $ 1604.142 (\pm 301.232)$ \\
  Wiki & GCN & EGO & $n.a.$ & $n.a.$ \\
  Wiki & GCN & CFF & $ 9.206 (\pm 0.466)$ & $ 1815.166 (\pm 236.533)$ \\
  Wiki & GCN & Combinex & $ 8.209 (\pm 0.589)$ & $ 3535.499 (\pm 1100.665)$ \\
  Wiki & GCN & UNR & $n.a.$ & $n.a.$ \\
  Facebook & GCN & CF-GNN & $n.a.$ & $ 1656.108 (\pm 119.632)$ \\
  Facebook & GCN & Random F. & $n.a.$ & $ 1503.831 (\pm 165.170)$ \\
  Facebook & GCN & Random E. & $ 1.348 (\pm 0.014)$ & $ 1495.108 (\pm 148.635)$ \\
  Facebook & GCN & EGO & $n.a.$ & $n.a.$ \\
  Facebook & GCN & CFF & $n.a.$ & $ 1751.805 (\pm 117.447)$ \\
  Facebook & GCN & Combinex & $ 8.178 (\pm 0.262)$ & $ 1744.821 (\pm 105.830)$ \\
  cora & GCN & CF-GNN & $ 4.778 (\pm 0.291)$ & $ 1422.808 (\pm 83.544)$ \\
  cora & GCN & Random F. & $ 1.338 (\pm 0.085)$ & $ 1354.186 (\pm 149.502)$ \\
  cora & GCN & Random E. & $ 1.317 (\pm 0.021)$ & $ 1341.519 (\pm 144.753)$ \\
  cora & GCN & EGO & $ 0.010 (\pm 0.003)$ & $n.a.$ \\
  cora & GCN & CFF & $n.a.$ & $ 1442.508 (\pm 61.366)$ \\
  cora & GCN & Combinex & $ 7.948 (\pm 0.237)$ & $ 1551.119 (\pm 88.321)$ \\
  cora & GCN & UNR & $ 0.266 (\pm 0.327)$ & $n.a.$ \\
  citeseer & GCN & CF-GNN & $ 4.576 (\pm 0.306)$ & $ 1445.919 (\pm 88.096)$ \\
  citeseer & GCN & Random F. & $ 1.287 (\pm 0.025)$ & $ 1387.031 (\pm 151.101)$ \\
  citeseer & GCN & Random E. & $ 1.350 (\pm 0.017)$ & $ 1359.386 (\pm 144.630)$ \\
  citeseer & GCN & EGO & $n.a.$ & $n.a.$ \\
  citeseer & GCN & CFF & $n.a.$ & $ 1469.579 (\pm 64.606)$ \\
  citeseer & GCN & Combinex & $ 7.665 (\pm 0.245)$ & $ 1583.035 (\pm 97.627)$ \\
  citeseer & GCN & UNR & $ 0.069 (\pm 0.038)$ & $n.a.$ \\
  pubmed & GCN & CF-GNN & $ 4.859 (\pm 0.148)$ & $ 1793.613 (\pm 152.189)$ \\
  pubmed & GCN & Random F. & $ 1.269 (\pm 0.031)$ & $ 1818.149 (\pm 268.231)$ \\
  pubmed & GCN & Random E. & $ 1.333 (\pm 0.022)$ & $ 1653.723 (\pm 212.566)$ \\
  pubmed & GCN & EGO & $ 0.011 (\pm 0.002)$ & $n.a.$ \\
  pubmed & GCN & CFF & $ 8.936 (\pm 0.204)$ & $ 1967.803 (\pm 171.638)$ \\
  pubmed & GCN & Combinex & $ 8.034 (\pm 0.321)$ & $ 2214.627 (\pm 261.309)$ \\
  pubmed & GCN & UNR & $n.a.$ & $ 1514.237 (\pm 226.171)$ \\
  Texas & GCN & CF-GNN & $ 4.712 (\pm 0.272)$ & $ 1280.175 (\pm 113.796)$ \\
  Texas & GCN & Random F. & $ 1.281 (\pm 0.001)$ & $ 1078.275 (\pm 0.000)$ \\
  Texas & GCN & Random E. & $ 1.356 (\pm 0.110)$ & $ 1076.808 (\pm 0.000)$ \\
  Texas & GCN & EGO & $ 0.011 (\pm 0.003)$ & $n.a.$ \\
  Texas & GCN & CFF & $n.a.$ & $ 1312.104 (\pm 92.521)$ \\
  Texas & GCN & Combinex & $ 7.775 (\pm 0.235)$ & $ 1302.808 (\pm 98.271)$ \\
  Texas & GCN & UNR & $n.a.$ & $n.a.$ \\
  Cornell & GCN & CF-GNN & $ 4.409 (\pm 0.155)$ & $ 1293.182 (\pm 105.387)$ \\
  Cornell & GCN & Random F. & $ 1.286 (\pm 0.008)$ & $ 1076.808 (\pm 0.000)$ \\
  Cornell & GCN & Random E. & $ 1.332 (\pm 0.008)$ & $ 1078.275 (\pm 0.000)$ \\
  Cornell & GCN & EGO & $n.a.$ & $n.a.$ \\
  Cornell & GCN & CFF & $n.a.$ & $ 1320.497 (\pm 83.093)$ \\
  Cornell & GCN & Combinex & $ 7.694 (\pm 0.196)$ & $ 1314.708 (\pm 87.600)$ \\
  Cornell & GCN & UNR & $n.a.$ & $n.a.$ \\
\hline
\end{tabular}
\caption{Metrics for different explainers}
\end{table*}
